XLBoost-Geo: An IP Geolocation System Based on Extreme Landmark Boosting

IP geolocation aims at locating the geographical position of Internet devices, which plays an essential role in many Internet applications. In this field, a long-standing challenge is how to find a large number of highly-reliable landmarks, which is the key to improve the precision of IP geolocation. To this end, many efforts have been made, while many IP geolocation methods still suffer from unacceptable error distance because of the lack of landmarks. In this paper, we propose a novel IP geolocation system, named XLBoost-Geo, which focuses on enhancing the number and the density of highly reliable landmarks. The main idea is to extract location-indicating clues from web pages and locating the web servers based on the clues. Based on the landmarks, XLBoost-Geo is able to geolocate arbitrary IPs with little error distance. Specifically, we first design an entity extracting method based on a bidirectional LSTM neural network with a self-adaptive loss function (LSTM-Ada) to extract the location-indicating clues on web pages and then generate landmarks based on the clues. Then, by measurements on network latency and topology, we estimate the closest landmark and associate the coordinate of the landmark with the location of the target IP. The results of our experiments clearly validate the effectiveness and efficiency of the extracting method, the precision, number, coverage of the landmarks, and the precision of the IP geolocation. On RIPE Atlas nodes, XLBoost-Geo achieves 2,561m median error distance, which outperforms SLG and IPIP.

==> Sections/Discussion.tex <==
\section{Discussion}
% 定位精度的差距主要来源于两个方面：1）地标数量与密度 2）最近地标的确定
% 与structon和SLG比较地标挖掘的数量和密度
    % it is difficult to cover all possible key words. 
    % map will not contains all websites, 一般只收录主站，会漏掉很多没有实际地理坐标的BBS、业务网站、组织官网等（XLBoost-Geo可以通过抽取属主名定位到这些web servers）
    % landmarks group by zipcode, SLG 和 XLBoost-Geo对比
    
    % 比起正则，挖掘方法更高效（Structon）
    % 扫描全网的网站，而不是依赖地图收录的站点
    % 利用了更多的信息（机构名）
    
% 最近地标的确定
    % SLG 在定位过程中通过traceroute实时地测量目标与地标之间的间接时延，这种单次测量得到的时延是不可靠的，非常依赖于网络的稳定与探测器的部署密度。
    % XLBoost-Geo 通过长期

==> Sections/Related_Work.tex <==
\section{Related Work}
In this section, We introduce some typical literature and works that relate to our study. They mainly fall into two aspects: \textit{Entity Extraction} and \textit{IP Geolocation}. 

\subsection{Entity Extraction}
In our study, the landmark mining process relies heavily on the accuracy of location clues extracted from web pages. In other words, an efficient and reliable algorithm to extract accurate location clues plays an important role in our study. In our approach, we model the clue mining task to an entity extraction task, which targets at locating location clues in the textual content on web pages. In the past, Entity extraction has been widely studied by researchers. Traditional algorithms, e.g., Hidden Markov Model\cite{zhou2002named} and Conditional Random Fields (CRF)\cite{passos2014lexicon}, usually rely on high-quality hand-crafted features and well-designed models. Recently, with the fast development and popularity of deep learning, several neural network-based sequential token tagging techniques have been proposed to address entity extraction tasks, which requires little manual labor to do feature engineering but achieved better performance. For instance, Lample et al. combined bidirectional Long Short-Term Memory networks (Bi-LSTM) and CRF in a supervised learning setting\cite{lample2016neural}, and Chiu et al. used a hybrid Bi-LSTM and Convolutional Neural Network (CNN) to detect both word and character-level features\cite{chiu2016named}.

\subsection{IP Geolocation}
IP geolocation methods can be simply divided into two categories: 1) \textit{Data mining-based Methods} and 2) \textit{Measurement-based Methods}. Data mining based methods are measurement-independent and only rely on mining location clues in source data to locate a target IP. These methods are easy to implement but the precision and the coverage are limited by mining methods and the quality of the source data. Measurement-based methods, which rely on network measurements, are universally applicable to nodes that allow ICMP requests. These methods can cover more IPs than data mining-base methods but suffer from higher computational overhead.

% public sources
Moore et al.\cite{whois_geo} mine regional Internet registry databases(Whois databases) for the address of the organization of a target IP. 
% registry based method 的问题：地址记录的是机构总部
For example, According to the Whois records, 99.7\% of the IPs of Google are located in Mountain View, California, where Google's headquarters resides, while in the fact, 47\% out of 4000 sampled IPs are evidenced not located in Mountain View.

Since a domain name can contain different granular descriptions of geographic location information, like the abbreviation of a city, state, or country, by mining this information, the geographic location of the target device can be inferred. Based on this idea, GeoTrack\cite{ip2geo}, DRoP \cite{huffaker2014drop}, rDNS-Geo \cite{dan2018ip_by_dns} and HLOC \cite{scheitle2017hloc} mine location clues in domain names to estimate a location. GeoTrack regards the last-hop router's location as an approximation of the address location of the host under test. It can be seen that the grain of the geographic location information in the domain name and the distance between the target device and the last-hop router determine the positioning precision of this approach. Structon \cite{structon} uses regular expressions to extract address information from web pages. By mapping addresses to the corresponding IPs of the web servers, it generate hundreds of thousands of landmarks with city-level precision.

% proprietary sources
% 私有或者很难获取的数据，方法难以复现和应用到其他地区
GeoCluster \cite{ip2geo} uses the address prefixes(AP) in BGP routing tables to cluster IP addresses and then deduce the entire cluster by location information of a few hosts in a cluster. The location information is extracted from three sources, including login and registration information of Hotmail users, HTTP cookies of bCentral, and users' query of FooTV. Checkin-Geo \cite{checkin_geo} leverages the location data shared by users in location-sharing services and logs of user logins from PCs for real-time and accurate geolocation. Dan et al.\cite{ipgeo_query_log} generate a large ground-truth dataset using real-time global positioning data extracted from search engine logs. Using the dataset, they measure the accuracy of three commercial IP geolocation databases. Plus, they introduce a technique to improve existing geolocation databases by mining explicit locations from query logs. Lee et al.\cite{lee2016ip} propose an IP geolocation database creation method based on a crowd-sourcing Internet broadband performance measurement tagged with locations and present an IP geolocation database based on 7 years of Internet broadband performance data in Korea.

\subsubsection{Measurement-based Methods}

GeoPing \cite{ip2geo} maps a node to a probe's location based on the measured delays from probes to the node. CBG \cite{cbg} utilizes measured delays and delay-distance relation to draw a set of constraints to narrow down the possible region that a target IP resides. TBG \cite{tbg} proves that network topology can be effectively used to achieve high geolocation accuracy. Octant \cite{octant} takes both positive and negative measurement constraints into account. Ciavarrini et al.\cite{ciavarrini2015geolocation}\cite{ciavarrini2017smartphone} devised an active IP geolocation method that uses smartphones as landmarks based on crowd-sourcing principles: a number of users participate voluntarily to the system and provide their devices as measuring elements. 

SLG \cite{wanggeo} utilizes zip codes on web pages to generate landmarks. An important contribution of this work lies in introducing a method that indirectly estimates the delay between a target and a landmark by finding the closest common router.

% 要分两段，延迟测量和引入拓扑的测量
% TBG和Octant依赖active landmarks(probes)
% SLG等依赖passive landmarks
% 

% 改进delay-distance model
\textbf{Probability and Statistics Based Methods:} Probability and statistics-based methods aim to study the relation between network delay and great circle distance and decrease the error introduced by the delay-distance model. Typical algorithms based on probability and statistics mainly include Posit\cite{eriksson2012posit}, Spotter\cite{laki2011spotter}, GBLC\cite{zhu2016city}, etc. They do not assume that there is a linear relationship between network delay and geographical distance but estimate the statistical relationship between them through statistical analysis of delay-distance data. The advantages of such algorithms are that they can reduce the Impact of inaccurate single delay measurement. However, the relationship between delay and geographical distance is inherently weak and heavily unreliable no matter what model is used to fit. First, the Internet consists of heterogeneous links, hosts, and routers whose transmission and processing speeds vary widely. Second, inelastic delays incurred on the last hop can introduce additional latencies that break the correspondence between round trip timings and physical distances. Finally, packets often follow indirect, circuitous paths from a source to a destination, rendering great-circle approximations inaccurate. Therefore, comparing with algorithms using a linear relationship, e.g. CBG, these methods improve little performance on IP geolocation and only achieve city-level precision.

% 将定位问题建模成机器学习问题
\textbf{Machine Learning Based Methods:} The main idea of Machine learning based methods is to reduce IP geolocation to a machine-learning classification problem. Typical machine learning based methods includes LBG\cite{eriksson2010learning}, ELC\cite{maziku2012enhancing}, CBIG\cite{biswal2014classification}, and NN-Geo\cite{jiang2016ip}. LBG\cite{eriksson2010learning} develops a Naive Bayes estimation method that assigns a given IP target to a geographic partition based on a set of lightweight measurements from a set of known monitors to the target. Specifically, two network measurements, latency and hop count, and a non-network measurement, population density, are considered as features. ELC\cite{maziku2012enhancing} extends LBG by extracting six features(average delay, standard deviation delay, mode delay, median delay, hop count, and population density), from measurements and implementing a new landmark selection policy. CBIG\cite{biswal2014classification} employs ELC to impove the accuracy of geolocating data files in datacenters in four commercial cloud providers. Experimental results show that high classification accuracy is obtained by using only three features (average delay, standard deviation delay, and hop count). The remaining three features did not significantly improve the accuracy of geolocation. With measurement results collected from these landmarks, Jiang et al.\cite{jiang2016ip} trained a two-tier neural network that estimated the geolocation of arbitrary IP addresses. In tier one, they use a radial basis function network(RBF) to find the region where the IP resides. In tier two, they use a multi-layer perceptron(MLP) to do a more precise estimation that focuses only on the region. On a dataset of 1,547 landmarks within the United States, the estimated median error distance is 4.1 kilometers.

